The $A_{inf}$-cohomology in the semistable case

For a proper, smooth scheme $X$ over a $p$-adic field $K$, we show that any proper, flat, semistable $\mathcal{O}_K$-model $\mathcal{X}$ of $X$ whose logarithmic de Rham cohomology is torsion free determines the same $\mathcal{O}_K$-lattice inside $H^i_{dR}(X/K)$ and, moreover, that this lattice is functorial in $X$. For this, we extend the results of Bhatt--Morrow--Scholze on the construction and the analysis of an $A_{inf}$-valued cohomology theory of $p$-adic formal, proper, smooth $\mathcal{O}_{\overline{K}}$-schemes $\mathfrak{X}$ to the semistable case. The relation of the $A_{inf}$-cohomology to the $p$-adic \'{e}tale and the logarithmic crystalline cohomologies allows us to reprove the semistable conjecture of Fontaine--Jannsen.

==> Omega.tex <==
% !TEX root = Ainf-coho.tex

\begin{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{The auxiliary object $\wt{\Omega}_\fX$ and its cohomology} \lab{OmegaX}

\revise{
%In \S\ref{AOmegaX}, we will relate $A\Omega_\fX$ to the logarithmic de Rham cohomology of $\fX$, and this will rest on an auxiliary object $\wt{\Omega}_\fX$, which we analyze in this section. For this, we loosely follow \cite{BMS16}*{\S8}, the key input to the \'{e}tale local analysis of $\wt{\Omega}_\fX$ being the almost purity theorem applied to a suitable perfectoid cover constructed with the help of an \'{e}tale local coordinate morphism \eqref{sst-coord}.  there are two key complications.

%Firstly, over the singular points, the layers of the perfectoid cover are no longer $\fX$-flat, which complicates transfer of continuous cohomology computations across the map \eqref{sst-coord} (contrast this with \cite{BMS16}*{proof of Prop.~8.9}). We bypass this issue by using results of Gabber--Ramero from \cite{GR03} to ensure that the map \eqref{sst-coord} is nevertheless flat.  
Secondly, the local comparison of $H^1(\wt{\Omega}_\fX)$ to K\"{a}hler differentials \emph{a priori} only applies on the smooth locus. To extend it to the singular locus, we proceed indirectly by bootstrapping from the smooth locus (see the proof of \Cref{Hi-OmegaX}).
%: in the proof , we first reduce to the case when $\fX$ is proper and algebraizable, then use non-Noetherian formal GAGA due to K.~Fujiwara and F.~Kato to algebraize a suitable comparison map, we then use results from \cite{Sch13} to analyze this map after inverting $p$, and we conclude , which is possible because $\cX$ is (S$_2$) and $\cX\setminus \cX^\sm$ is of codimension $\ge 2$ in $\cX$.

%We begin by defining the object $\wt{\Omega}_\fX$ that we are going to study.



























%\brem \lab{dR-iso-uniq}
%By the proof above, we may (and do) choose the isomorphism \eqref{Hi-OmegaX-eq} in such a way that its restriction to $\fX^\sm$ is compatible with the analogous isomorphism constructed in \cite{BMS16}*{8.3} in the smooth case. This compatibility determines the isomorphism \eqref{Hi-OmegaX-eq} uniquely.
%\remi
%In \Cref{Hi-OmegaX}, we assumed that $\cX$ is proper in order to avoid analyzing the map \eqref{omg-comp-map} at the singular points. We expect that \eqref{Hi-OmegaX-eq} also holds without the properness assumption.  
%\erem
}





\end{document}
